Diffusion models meet image counter-forensics

From its acquisition in the camera sensors to its storage, different operations are performed to generate the final image. This pipeline imprints specific traces into the image to form a natural watermark. Tampering with an image disturbs these traces; these disruptions are clues that are used by most methods to detect and locate forgeries. In this article, we assess the capabilities of diffusion models to erase the traces left by forgers and, therefore, deceive forensics methods. Such an approach has been recently introduced for adversarial purification, achieving significant performance. We show that diffusion purification methods are well suited for counter-forensics tasks. Such approaches outperform already existing counter-forensics techniques both in deceiving forensics methods and in preserving the natural look of the purified images. The source code is publicly available at https://github.com/mtailanian/diff-cf.

==> tables/all-mcc-iou-grayout.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}


\begin{table*}[t]  
  \small  
  \centering
  \setlength{\tabcolsep}{0em}
  \begin{tabularx}{1\textwidth}{c@{\hskip 3pt}l@{\hskip 3pt}lllllllllc}

\toprule

 & & CatNet & Choi & Comprint & MantraNet & Noiseprint & Shin & SpliceBuster & TruFor & ZERO & Avg$_w$ diff.\\ 
\midrule

\multirow{10}{*}[.4em]{\rotatebox[origin=c]{90}{\footnotesize{Korus  }}} & \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Original}}} &\gomcc{ 0.0790  }&\mcc{ 0.1971  }&\gomcc{ 0.0534  }&\mcc{ 0.1261  }&\mcc{ 0.0988  }&\gomcc{ 0.0221  }&\mcc{ 0.1405  }&\mcc{ 0.3428  } & \gomcc{0.0050} & - \\

& &\goiou{ 0.0433  }&\iou{ 0.1261  }&\goiou{ 0.0461  }&\iou{ 0.0982  }&\iou{ 0.0792  }&\goiou{ 0.0568  }&\iou{ 0.1012  }&\iou{ 0.2575  } & \goiou{0.0028} & -\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{CamTE}}} &\gomcc{ 0.0468 \tiny{(-0.0322)} }&\mcc{ 0.0597 \tiny{(-0.1374)} }&\gomcc{ 0.0356 \tiny{(-0.0179)} }&\mcc{ 0.0646 \tiny{(-0.0614)} }&\mcc{ 0.0420 \tiny{(-0.0569)} }&\gomcc{ 0.0305 \tiny{(0.0084)} }&\mcc{ 0.0817 \tiny{(-0.0588)} }&\mcc{ 0.1961 \tiny{(-0.1467)} } & \gomcc{0.0000 \tiny{(-0.0050)}} & \mcc{-0.1024}\\
& &\goiou{ 0.0278 \tiny{(-0.0155)} }&\iou{ 0.0400 \tiny{(-0.0860)} }&\goiou{ 0.0389 \tiny{(-0.0072)} }&\iou{ 0.0644 \tiny{(-0.0338)} }&\iou{ 0.0545 \tiny{(-0.0247)} }&\goiou{ 0.0578 \tiny{(0.0011)} }&\iou{ 0.0729 \tiny{(-0.0284)} }&\iou{ 0.1489 \tiny{(-0.1086)} } & \goiou{0.0000 \tiny{(-0.0028)}} & \iou{-0.0479}\\


& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{BM3D}}} &\gomcc{ 0.0997 \tiny{(0.0207)} }&\mcc{ 0.0352 \tiny{(-0.1619)} }&\gomcc{ 0.0278 \tiny{(-0.0256)} }&\mcc{ 0.0652 \tiny{(-0.0609)} }&\mcc{ 0.0420 \tiny{(-0.0569)} }&\gomcc{ 0.0155 \tiny{(-0.0066)} }&\mcc{ 0.0860 \tiny{(-0.0545)} }&\mcc{ 0.2579 \tiny{(-0.0850)} } & \gomcc{0.0000 \tiny{(-0.0050)}} & \mcc{-0.0819}\\
& &\goiou{ 0.0646 \tiny{(0.0213)} }&\iou{ 0.0227 \tiny{(-0.1033)} }&\goiou{ 0.0346 \tiny{(-0.0115)} }&\iou{ 0.0746 \tiny{(-0.0237)} }&\iou{ 0.0514 \tiny{(-0.0278)} }&\goiou{ 0.0540 \tiny{(-0.0028)} }&\iou{ 0.0744 \tiny{(-0.0268)} }&\iou{ 0.1964 \tiny{(-0.0611)} } & \goiou{0.0000 \tiny{(-0.0028)}} & \iou{-0.0358}\\


& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Diff-CF}}} &\gomcc{ 0.0418 \tiny{(-0.0371)} }&\mcc{ 0.0147 \tiny{(-0.1825)} }&\gomcc{ 0.0024 \tiny{(-0.0510)} }&\mcc{ 0.0255 \tiny{(-0.1005)} }&\mcc{ 0.0190 \tiny{(-0.0798)} }&\gomcc{ 0.0027 \tiny{(-0.0194)} }&\mcc{ 0.0350 \tiny{(-0.1055)} }&\mcc{ 0.1454 \tiny{(-0.1974)} } & \gomcc{0.0045 \tiny{(-0.0005)}} & \mccb{-0.1451}\\
& &\goiou{ 0.0204 \tiny{(-0.0229)} }&\iou{ 0.0246 \tiny{(-0.1014)} }&\goiou{ 0.0215 \tiny{(-0.0246)} }&\iou{ 0.0416 \tiny{(-0.0566)} }&\iou{ 0.0360 \tiny{(-0.0432)} }&\goiou{ 0.0487 \tiny{(-0.0081)} }&\iou{ 0.0401 \tiny{(-0.0611)} }&\iou{ 0.1131 \tiny{(-0.1445)} } & \goiou{0.0027 \tiny{(-0.0001)}} & \ioub{-0.0677}\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Diff-CFG}}} &\gomcc{ 0.0852 \tiny{(0.0063)} }&\mcc{ 0.0044 \tiny{(-0.1927)} }&\gomcc{ 0.0125 \tiny{(-0.0409)} }&\mcc{ 0.0442 \tiny{(-0.0818)} }&\mcc{ 0.0267 \tiny{(-0.0722)} }&\gomcc{ 0.0040 \tiny{(-0.0181)} }&\mcc{ 0.0456 \tiny{(-0.0950)} }&\mcc{ 0.2064 \tiny{(-0.1364)} } & \gomcc{0.0005 \tiny{(-0.0045)}} & \mccb{-0.1177} \\
& &\goiou{ 0.0527 \tiny{(0.0095)} }&\iou{ 0.0043 \tiny{(-0.1217)} }&\goiou{ 0.0281 \tiny{(-0.0180)} }&\iou{ 0.0552 \tiny{(-0.0430)} }&\iou{ 0.0446 \tiny{(-0.0346)} }&\goiou{ 0.0491 \tiny{(-0.0076)} }&\iou{ 0.0488 \tiny{(-0.0525)} }&\iou{ 0.1601 \tiny{(-0.0975)} }& \goiou{0.0011 \tiny{(-0.0017)}} & \ioub{-0.0536}\\

\midrule

\multirow{10}{*}[.4em]{\rotatebox[origin=c]{90}{\footnotesize{FAU  }}} & \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Original}}} &\mcc{ 0.3228  }&\mcc{ 0.3045  }&\mcc{ 0.0393  }&\gomcc{ 0.0203  }&\mcc{ 0.0358  }&\mcc{ 0.1134  }&\mcc{ 0.0074  }&\mcc{ 0.4039  }&\mcc{ 0.2757 }\\
& &\iou{ 0.2329  }&\iou{ 0.2670  }&\iou{ 0.0305  }&\goiou{ 0.0336  }&\iou{ 0.0482  }&\iou{ 0.1289  }&\iou{ 0.0251  }&\iou{ 0.3373  }&\iou{ 0.2021} & - \\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{CamTE}}} &\mcc{ 0.0141 \tiny{(-0.3087)} }&\mcc{ 0.1426 \tiny{(-0.1620)} }&\mcc{ 0.0092 \tiny{(-0.0302)} }&\gomcc{ 0.0154 \tiny{(-0.0049)} }&\mcc{ 0.0242 \tiny{(-0.0116)} }&\mcc{ 0.0826 \tiny{(-0.0308)} }&\mcc{ 0.0045 \tiny{(-0.0029)} }&\mcc{ 0.0553 \tiny{(-0.3486)} }&\mcc{ -0.0010 \tiny{(-0.2767)}} & \mcc{-0.3713}\\
& &\iou{ 0.0085 \tiny{(-0.2244)} }&\iou{ 0.1173 \tiny{(-0.1497)} }&\iou{ 0.0206 \tiny{(-0.0099)} }&\goiou{ 0.0427 \tiny{(0.0091)} }&\iou{ 0.0434 \tiny{(-0.0049)} }&\iou{ 0.1046 \tiny{(-0.0243)} }&\iou{ 0.0277 \tiny{(0.0026)} }&\iou{ 0.0572 \tiny{(-0.2801)} }&\iou{ 0.0633 \tiny{(-0.1388)}} & \iou{-0.2181}\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{BM3D}}} &\mcc{ 0.0757 \tiny{(-0.2471)} }&\mcc{ 0.0679 \tiny{(-0.2367)} }&\mcc{ -0.0017 \tiny{(-0.0410)} }&\gomcc{ -0.0268 \tiny{(-0.0470)} }&\mcc{ -0.0014 \tiny{(-0.0372)} }&\mcc{ 0.0411 \tiny{(-0.0723)} }&\mcc{ 0.0011 \tiny{(-0.0064)} }&\mcc{ 0.0802 \tiny{(-0.3237)} }&\mcc{ -0.0114 \tiny{(-0.2871)}} & \mcc{-0.3739}\\
& &\iou{ 0.0517 \tiny{(-0.1812)} }&\iou{ 0.0559 \tiny{(-0.2111)} }&\iou{ 0.0126 \tiny{(-0.0179)} }&\goiou{ 0.0377 \tiny{(0.0041)} }&\iou{ 0.0331 \tiny{(-0.0152)} }&\iou{ 0.0803 \tiny{(-0.0486)} }&\iou{ 0.0243 \tiny{(-0.0008)} }&\iou{ 0.0799 \tiny{(-0.2574)} }&\iou{ 0.0583 \tiny{(-0.1438)}} & \iou{-0.2219}\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Diff-CF}}} &\mcc{ 0.0070 \tiny{(-0.3157)} }&\mcc{ 0.0242 \tiny{(-0.2803)} }&\mcc{ 0.0001 \tiny{(-0.0392)} }&\gomcc{ 0.0057 \tiny{(-0.0146)} }&\mcc{ -0.0018 \tiny{(-0.0376)} }&\mcc{ 0.0128 \tiny{(-0.1006)} }&\mcc{ -0.0050 \tiny{(-0.0124)} }&\mcc{ 0.0399 \tiny{(-0.3640)} }&\mcc{ -0.0007 \tiny{(-0.2765)}} & \mccb{-0.4252}\\
& &\iou{ 0.0056 \tiny{(-0.2273)} }&\iou{ 0.0458 \tiny{(-0.2213)} }&\iou{ 0.0159 \tiny{(-0.0146)} }&\goiou{ 0.0355 \tiny{(0.0019)} }&\iou{ 0.0199 \tiny{(-0.0283)} }&\iou{ 0.0602 \tiny{(-0.0687)} }&\iou{ 0.0123 \tiny{(-0.0128)} }&\iou{ 0.0520 \tiny{(-0.2853)} }&\iou{ 0.0015 \tiny{(-0.2006)}} & \ioub{-0.2597}\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Diff-CFG}}} &\mcc{ 0.0241 \tiny{(-0.2986)} }&\mcc{ 0.0137 \tiny{(-0.2908)} }&\mcc{ -0.0059 \tiny{(-0.0452)} }&\gomcc{ 0.0128 \tiny{(-0.0075)} }&\mcc{ 0.0002 \tiny{(-0.0355)} }&\mcc{ 0.0202 \tiny{(-0.0933)} }&\mcc{ 0.0127 \tiny{(0.0053)} }&\mcc{ 0.0470 \tiny{(-0.3569)} }&\mcc{ -0.0043 \tiny{(-0.2800)}} & \mccb{-0.4200}\\
& &\iou{ 0.0184 \tiny{(-0.2145)} }&\iou{ 0.0220 \tiny{(-0.2451)} }&\iou{ 0.0143 \tiny{(-0.0162)} }&\goiou{ 0.0339 \tiny{(0.0003)} }&\iou{ 0.0287 \tiny{(-0.0196)} }&\iou{ 0.0646 \tiny{(-0.0643)} }&\iou{ 0.0246 \tiny{(-0.0005)} }&\iou{ 0.0592 \tiny{(-0.2781)} }&\iou{ 0.0008 \tiny{(-0.2012)}} & \ioub{-0.2596}\\

\midrule

\multirow{10}{*}[.4em]{\rotatebox[origin=c]{90}{\footnotesize{COVERAGE  }}} 

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Original}}} &
   \mcc{ 0.2747  }&\mcc{ 0.0075  }&\mcc{ 0.0230 }&\mcc{0.2617 }&\mcc{ 0.0062 }&\mcc{ 0.0615   }&\mcc{ -0.0571  }&\mcc{ 0.4442}&\mcc{ 0.0326 } & -\\
& &\iou{0.2199                 } & \iou{0.0109                 } & \iou{0.0856                 } & \iou{0.1856                 } & \iou{0.0858                 } & \iou{0.1106                 } & \iou{0.0423                 } & \iou{0.3752                 } & \iou{0.1082                 } & - \\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{CamTE}}} 
  &\mcc{0.1480 \tiny{(-0.1267)}} & \mcc{0.0056  \tiny{(-0.0020)}} & \mcc{-0.0015 \tiny{(-0.0245)}} & \mcc{0.0790 \tiny{(-0.1827)}} & \mcc{-0.0230 \tiny{(-0.0292)}} & \mcc{0.0489 \tiny{(-0.0127)}} & \mcc{-0.0722 \tiny{(-0.0151)}} & \mcc{0.2614 \tiny{(-0.1828)}} & \mcc{0.0238 \tiny{(-0.0088)}} & \mccb{-0.1648} \\
& &\iou{0.1162 \tiny{(-0.1038)}} & \iou{0.0079 \tiny{(-0.0030)}} & \iou{0.0711 \tiny{(-0.0145)}} & \iou{0.0719 \tiny{(-0.1137)}} & \iou{0.0770 \tiny{(-0.0089)}} & \iou{0.1043 \tiny{(-0.0063)}} & \iou{0.0361 \tiny{(-0.0062)}} & \iou{0.2212 \tiny{(-0.1541)}} & \iou{0.1046 \tiny{(-0.0036)}} & \ioub{-0.1051} \\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{BM3D}}} 
  &\mcc{0.2666 \tiny{(-0.0081)}} & \mcc{0.0051  \tiny{(-0.0024)}} & \mcc{-0.0281 \tiny{(-0.0511)}} & \mcc{0.0371 \tiny{(-0.2246)}} & \mcc{-0.0145 \tiny{(-0.0207)}} & \mcc{0.0515 \tiny{(-0.0100)}} & \mcc{-0.0771 \tiny{(-0.0200)}} & \mcc{0.3267 \tiny{(-0.1175)}} & \mcc{0.0236 \tiny{(-0.0091)}} & \mcc{-0.1143}\\
& &\iou{0.2151 \tiny{(-0.0049)}} & \iou{0.0036 \tiny{(-0.0072)}} & \iou{0.0617 \tiny{(-0.0240)}} & \iou{0.0841 \tiny{(-0.1015)}} & \iou{0.0773 \tiny{(-0.0085)}} & \iou{0.1055 \tiny{(-0.0051)}} & \iou{0.0336 \tiny{(-0.0087)}} & \iou{0.2863 \tiny{(-0.0889)}} & \iou{0.1046 \tiny{(-0.0036)}} & \iou{-0.0575} \\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Diff-CF}}} 
  &\mcc{0.1598 \tiny{(-0.1149)}} & \mcc{0.0011  \tiny{(-0.0064)}} & \mcc{-0.0065 \tiny{(-0.0295)}} & \mcc{0.0483 \tiny{(-0.2133)}} & \mcc{-0.0115 \tiny{(-0.0176)}} & \mcc{0.0514 \tiny{(-0.0101)}} & \mcc{-0.0602 \tiny{(-0.0031)}} & \mcc{0.2849 \tiny{(-0.1594)}} & \mcc{0.0000 \tiny{(-0.0326)}} & \mccb{-0.1605}\\
& &\iou{0.1278 \tiny{(-0.0922)}} & \iou{0.0059 \tiny{(-0.0050)}} & \iou{0.0687 \tiny{(-0.0169)}} & \iou{0.0537 \tiny{(-0.1320)}} & \iou{0.0790 \tiny{(-0.0068)}} & \iou{0.1055 \tiny{(-0.0051)}} & \iou{0.0383 \tiny{(-0.0040)}} & \iou{0.2427 \tiny{(-0.1325)}} & \iou{0.0000 \tiny{(-0.1082)}} & \ioub{-0.1090} \\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Diff-CFG}}} 
  &\mcc{0.2003 \tiny{(-0.0745)}} & \mcc{-0.0004 \tiny{(-0.0079)}} & \mcc{-0.0124 \tiny{(-0.0354)}} & \mcc{0.0680 \tiny{(-0.1937)}} & \mcc{0.0024 \tiny{(-0.0038)} } & \mcc{0.0475 \tiny{(-0.0140)}} & \mcc{-0.0717 \tiny{(-0.0146)}} & \mcc{0.2738 \tiny{(-0.1704)}} & \mcc{0.0000 \tiny{(-0.0326)}} & \mcc{-0.1488}\\
& &\iou{0.1607 \tiny{(-0.0592)}} & \iou{0.0010 \tiny{(-0.0099)}} & \iou{0.0630 \tiny{(-0.0226)}} & \iou{0.0693 \tiny{(-0.1163)}} & \iou{0.0858 \tiny{(0.0000)} } & \iou{0.1051 \tiny{(-0.0055)}} & \iou{0.0334 \tiny{(-0.0090)}} & \iou{0.2386 \tiny{(-0.1367)}} & \iou{0.0000 \tiny{(-0.1082)}} & \iou{-0.1006} \\

\bottomrule
  \end{tabularx}
  \caption{All  datasets \mcc{mcc} and \iou{iou}}
  \label{tab:all-mcc-iou}
\end{table*}

==> tables/all-mcc-iou.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}


\begin{table*}[t]  
  \small  
  \centering
  \setlength{\tabcolsep}{0em}
  \begin{tabularx}{1\textwidth}{c@{\hskip 3pt}l@{\hskip 3pt}llllllllll}

\toprule

 & & CatNet & Bammey & Choi & Comprint & MantraNet & Noiseprint & Shin & SpliceBuster & TruFor & ZERO\\ 
\midrule

\multirow{10}{*}[.4em]{\rotatebox[origin=c]{90}{\footnotesize{Korus  }}} & \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Original}}} &\mcc{ 0.0790  }&\mcc{ -0.1548  }&\mcc{ 0.1971  }&\mcc{ 0.0534  }&\mcc{ 0.1261  }&\mcc{ 0.0988  }&\mcc{ 0.0221  }&\mcc{ 0.1405  }&\mcc{ 0.3428  } & -\\

& &\iou{ 0.0433  }&\iou{ 0.0446  }&\iou{ 0.1261  }&\iou{ 0.0461  }&\iou{ 0.0982  }&\iou{ 0.0792  }&\iou{ 0.0568  }&\iou{ 0.1012  }&\iou{ 0.2575  } & -\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{CamTE}}} &\mcc{ 0.0468 \tiny{(-0.0322)} }&\mcc{ -0.0608 \tiny{(0.0940)} }&\mcc{ 0.0597 \tiny{(-0.1374)} }&\mcc{ 0.0356 \tiny{(-0.0179)} }&\mcc{ 0.0646 \tiny{(-0.0614)} }&\mcc{ 0.0420 \tiny{(-0.0569)} }&\mcc{ 0.0305 \tiny{(0.0084)} }&\mcc{ 0.0817 \tiny{(-0.0588)} }&\mcc{ 0.1961 \tiny{(-0.1467)} } & -\\
& &\iou{ 0.0278 \tiny{(-0.0155)} }&\iou{ 0.0452 \tiny{(0.0005)} }&\iou{ 0.0400 \tiny{(-0.0860)} }&\iou{ 0.0389 \tiny{(-0.0072)} }&\iou{ 0.0644 \tiny{(-0.0338)} }&\iou{ 0.0545 \tiny{(-0.0247)} }&\iou{ 0.0578 \tiny{(0.0011)} }&\iou{ 0.0729 \tiny{(-0.0284)} }&\iou{ 0.1489 \tiny{(-0.1086)} } & -\\


& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{BM3D}}} &\mcc{ 0.0997 \tiny{(0.0207)} }&\mcc{ -0.0452 \tiny{(0.1095)} }&\mcc{ 0.0352 \tiny{(-0.1619)} }&\mcc{ 0.0278 \tiny{(-0.0256)} }&\mcc{ 0.0652 \tiny{(-0.0609)} }&\mcc{ 0.0420 \tiny{(-0.0569)} }&\mcc{ 0.0155 \tiny{(-0.0066)} }&\mcc{ 0.0860 \tiny{(-0.0545)} }&\mcc{ 0.2579 \tiny{(-0.0850)} } & -\\
& &\iou{ 0.0646 \tiny{(0.0213)} }&\iou{ 0.0478 \tiny{(0.0031)} }&\iou{ 0.0227 \tiny{(-0.1033)} }&\iou{ 0.0346 \tiny{(-0.0115)} }&\iou{ 0.0746 \tiny{(-0.0237)} }&\iou{ 0.0514 \tiny{(-0.0278)} }&\iou{ 0.0540 \tiny{(-0.0028)} }&\iou{ 0.0744 \tiny{(-0.0268)} }&\iou{ 0.1964 \tiny{(-0.0611)} } & -\\


& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Ricky}}} &\mcc{ 0.0418 \tiny{(-0.0371)} }&\mcc{ -0.0030 \tiny{(0.1518)} }&\mcc{ 0.0147 \tiny{(-0.1825)} }&\mcc{ 0.0024 \tiny{(-0.0510)} }&\mcc{ 0.0255 \tiny{(-0.1005)} }&\mcc{ 0.0190 \tiny{(-0.0798)} }&\mcc{ 0.0027 \tiny{(-0.0194)} }&\mcc{ 0.0350 \tiny{(-0.1055)} }&\mcc{ 0.1454 \tiny{(-0.1974)} } & -\\
& &\iou{ 0.0204 \tiny{(-0.0229)} }&\iou{ 0.0505 \tiny{(0.0059)} }&\iou{ 0.0246 \tiny{(-0.1014)} }&\iou{ 0.0215 \tiny{(-0.0246)} }&\iou{ 0.0416 \tiny{(-0.0566)} }&\iou{ 0.0360 \tiny{(-0.0432)} }&\iou{ 0.0487 \tiny{(-0.0081)} }&\iou{ 0.0401 \tiny{(-0.0611)} }&\iou{ 0.1131 \tiny{(-0.1445)} } & -\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{RickyG}}} &\mcc{ 0.0852 \tiny{(0.0063)} }&\mcc{ -0.0096 \tiny{(0.1452)} }&\mcc{ 0.0044 \tiny{(-0.1927)} }&\mcc{ 0.0125 \tiny{(-0.0409)} }&\mcc{ 0.0442 \tiny{(-0.0818)} }&\mcc{ 0.0267 \tiny{(-0.0722)} }&\mcc{ 0.0040 \tiny{(-0.0181)} }&\mcc{ 0.0456 \tiny{(-0.0950)} }&\mcc{ 0.2064 \tiny{(-0.1364)} }& -\\
& &\iou{ 0.0527 \tiny{(0.0095)} }&\iou{ 0.0495 \tiny{(0.0048)} }&\iou{ 0.0043 \tiny{(-0.1217)} }&\iou{ 0.0281 \tiny{(-0.0180)} }&\iou{ 0.0552 \tiny{(-0.0430)} }&\iou{ 0.0446 \tiny{(-0.0346)} }&\iou{ 0.0491 \tiny{(-0.0076)} }&\iou{ 0.0488 \tiny{(-0.0525)} }&\iou{ 0.1601 \tiny{(-0.0975)} }& -\\

\midrule
\multirow{10}{*}[.4em]{\rotatebox[origin=c]{90}{\footnotesize{FAU  }}} & \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Original}}} &\mcc{ 0.3228  }&\mcc{ -0.1696  }&\mcc{ 0.3045  }&\mcc{ 0.0393  }&\mcc{ 0.0203  }&\mcc{ 0.0358  }&\mcc{ 0.1134  }&\mcc{ 0.0074  }&\mcc{ 0.4039  }&\mcc{ 0.2757 }\\
& &\iou{ 0.2329  }&\iou{ 0.0469  }&\iou{ 0.2670  }&\iou{ 0.0305  }&\iou{ 0.0336  }&\iou{ 0.0482  }&\iou{ 0.1289  }&\iou{ 0.0251  }&\iou{ 0.3373  }&\iou{ 0.2021} \\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{CamTE}}} &\mcc{ 0.0141 \tiny{(-0.3087)} }&\mcc{ -0.0738 \tiny{(0.0958)} }&\mcc{ 0.1426 \tiny{(-0.1620)} }&\mcc{ 0.0092 \tiny{(-0.0302)} }&\mcc{ 0.0154 \tiny{(-0.0049)} }&\mcc{ 0.0242 \tiny{(-0.0116)} }&\mcc{ 0.0826 \tiny{(-0.0308)} }&\mcc{ 0.0045 \tiny{(-0.0029)} }&\mcc{ 0.0553 \tiny{(-0.3486)} }&\mcc{ -0.0010 \tiny{(-0.2767)}}\\
& &\iou{ 0.0085 \tiny{(-0.2244)} }&\iou{ 0.0516 \tiny{(0.0047)} }&\iou{ 0.1173 \tiny{(-0.1497)} }&\iou{ 0.0206 \tiny{(-0.0099)} }&\iou{ 0.0427 \tiny{(0.0091)} }&\iou{ 0.0434 \tiny{(-0.0049)} }&\iou{ 0.1046 \tiny{(-0.0243)} }&\iou{ 0.0277 \tiny{(0.0026)} }&\iou{ 0.0572 \tiny{(-0.2801)} }&\iou{ 0.0633 \tiny{(-0.1388)}}\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{BM3D}}} &\mcc{ 0.0757 \tiny{(-0.2471)} }&\mcc{ -0.0692 \tiny{(0.1004)} }&\mcc{ 0.0679 \tiny{(-0.2367)} }&\mcc{ -0.0017 \tiny{(-0.0410)} }&\mcc{ -0.0268 \tiny{(-0.0470)} }&\mcc{ -0.0014 \tiny{(-0.0372)} }&\mcc{ 0.0411 \tiny{(-0.0723)} }&\mcc{ 0.0011 \tiny{(-0.0064)} }&\mcc{ 0.0802 \tiny{(-0.3237)} }&\mcc{ -0.0114 \tiny{(-0.2871)}}\\
& &\iou{ 0.0517 \tiny{(-0.1812)} }&\iou{ 0.0517 \tiny{(0.0048)} }&\iou{ 0.0559 \tiny{(-0.2111)} }&\iou{ 0.0126 \tiny{(-0.0179)} }&\iou{ 0.0377 \tiny{(0.0041)} }&\iou{ 0.0331 \tiny{(-0.0152)} }&\iou{ 0.0803 \tiny{(-0.0486)} }&\iou{ 0.0243 \tiny{(-0.0008)} }&\iou{ 0.0799 \tiny{(-0.2574)} }&\iou{ 0.0583 \tiny{(-0.1438)}}\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Ricky}}} &\mcc{ 0.0070 \tiny{(-0.3157)} }&\mcc{ -0.0130 \tiny{(0.1567)} }&\mcc{ 0.0242 \tiny{(-0.2803)} }&\mcc{ 0.0001 \tiny{(-0.0392)} }&\mcc{ 0.0057 \tiny{(-0.0146)} }&\mcc{ -0.0018 \tiny{(-0.0376)} }&\mcc{ 0.0128 \tiny{(-0.1006)} }&\mcc{ -0.0050 \tiny{(-0.0124)} }&\mcc{ 0.0399 \tiny{(-0.3640)} }&\mcc{ -0.0007 \tiny{(-0.2765)}}\\
& &\iou{ 0.0056 \tiny{(-0.2273)} }&\iou{ 0.0548 \tiny{(0.0079)} }&\iou{ 0.0458 \tiny{(-0.2213)} }&\iou{ 0.0159 \tiny{(-0.0146)} }&\iou{ 0.0355 \tiny{(0.0019)} }&\iou{ 0.0199 \tiny{(-0.0283)} }&\iou{ 0.0602 \tiny{(-0.0687)} }&\iou{ 0.0123 \tiny{(-0.0128)} }&\iou{ 0.0520 \tiny{(-0.2853)} }&\iou{ 0.0015 \tiny{(-0.2006)}}\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{RickyG}}} &\mcc{ 0.0241 \tiny{(-0.2986)} }&\mcc{ -0.0243 \tiny{(0.1453)} }&\mcc{ 0.0137 \tiny{(-0.2908)} }&\mcc{ -0.0059 \tiny{(-0.0452)} }&\mcc{ 0.0128 \tiny{(-0.0075)} }&\mcc{ 0.0002 \tiny{(-0.0355)} }&\mcc{ 0.0202 \tiny{(-0.0933)} }&\mcc{ 0.0127 \tiny{(0.0053)} }&\mcc{ 0.0470 \tiny{(-0.3569)} }&\mcc{ -0.0043 \tiny{(-0.2800)}}\\
& &\iou{ 0.0184 \tiny{(-0.2145)} }&\iou{ 0.0536 \tiny{(0.0067)} }&\iou{ 0.0220 \tiny{(-0.2451)} }&\iou{ 0.0143 \tiny{(-0.0162)} }&\iou{ 0.0339 \tiny{(0.0003)} }&\iou{ 0.0287 \tiny{(-0.0196)} }&\iou{ 0.0646 \tiny{(-0.0643)} }&\iou{ 0.0246 \tiny{(-0.0005)} }&\iou{ 0.0592 \tiny{(-0.2781)} }&\iou{ 0.0008 \tiny{(-0.2012)}}\\

\midrule



\multirow{10}{*}[.4em]{\rotatebox[origin=c]{90}{\footnotesize{COVERAGE  }}} & \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Original}}} &\mcc{ 0.3228  }&\mcc{ -0.1696  }&\mcc{ 0.3045  }&\mcc{ 0.0393  }&\mcc{ 0.0203  }&\mcc{ 0.0358  }&\mcc{ 0.1134  }&\mcc{ 0.0074  }&\mcc{ 0.4039  }&\mcc{ 0.2757 }\\
& &\iou{ 0.2329  }&\iou{ 0.0469  }&\iou{ 0.2670  }&\iou{ 0.0305  }&\iou{ 0.0336  }&\iou{ 0.0482  }&\iou{ 0.1289  }&\iou{ 0.0251  }&\iou{ 0.3373  }&\iou{ 0.2021} \\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{CamTE}}} &\mcc{ 0.0141 \tiny{(-0.3087)} }&\mcc{ -0.0738 \tiny{(0.0958)} }&\mcc{ 0.1426 \tiny{(-0.1620)} }&\mcc{ 0.0092 \tiny{(-0.0302)} }&\mcc{ 0.0154 \tiny{(-0.0049)} }&\mcc{ 0.0242 \tiny{(-0.0116)} }&\mcc{ 0.0826 \tiny{(-0.0308)} }&\mcc{ 0.0045 \tiny{(-0.0029)} }&\mcc{ 0.0553 \tiny{(-0.3486)} }&\mcc{ -0.0010 \tiny{(-0.2767)}}\\
& &\iou{ 0.0085 \tiny{(-0.2244)} }&\iou{ 0.0516 \tiny{(0.0047)} }&\iou{ 0.1173 \tiny{(-0.1497)} }&\iou{ 0.0206 \tiny{(-0.0099)} }&\iou{ 0.0427 \tiny{(0.0091)} }&\iou{ 0.0434 \tiny{(-0.0049)} }&\iou{ 0.1046 \tiny{(-0.0243)} }&\iou{ 0.0277 \tiny{(0.0026)} }&\iou{ 0.0572 \tiny{(-0.2801)} }&\iou{ 0.0633 \tiny{(-0.1388)}}\\


& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{BM3D}}} &\mcc{ 0.0757 \tiny{(-0.2471)} }&\mcc{ -0.0692 \tiny{(0.1004)} }&\mcc{ 0.0679 \tiny{(-0.2367)} }&\mcc{ -0.0017 \tiny{(-0.0410)} }&\mcc{ -0.0268 \tiny{(-0.0470)} }&\mcc{ -0.0014 \tiny{(-0.0372)} }&\mcc{ 0.0411 \tiny{(-0.0723)} }&\mcc{ 0.0011 \tiny{(-0.0064)} }&\mcc{ 0.0802 \tiny{(-0.3237)} }&\mcc{ -0.0114 \tiny{(-0.2871)}}\\
& &\iou{ 0.0517 \tiny{(-0.1812)} }&\iou{ 0.0517 \tiny{(0.0048)} }&\iou{ 0.0559 \tiny{(-0.2111)} }&\iou{ 0.0126 \tiny{(-0.0179)} }&\iou{ 0.0377 \tiny{(0.0041)} }&\iou{ 0.0331 \tiny{(-0.0152)} }&\iou{ 0.0803 \tiny{(-0.0486)} }&\iou{ 0.0243 \tiny{(-0.0008)} }&\iou{ 0.0799 \tiny{(-0.2574)} }&\iou{ 0.0583 \tiny{(-0.1438)}}\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{Ricky}}} &\mcc{ 0.0070 \tiny{(-0.3157)} }&\mcc{ -0.0130 \tiny{(0.1567)} }&\mcc{ 0.0242 \tiny{(-0.2803)} }&\mcc{ 0.0001 \tiny{(-0.0392)} }&\mcc{ 0.0057 \tiny{(-0.0146)} }&\mcc{ -0.0018 \tiny{(-0.0376)} }&\mcc{ 0.0128 \tiny{(-0.1006)} }&\mcc{ -0.0050 \tiny{(-0.0124)} }&\mcc{ 0.0399 \tiny{(-0.3640)} }&\mcc{ -0.0007 \tiny{(-0.2765)}}\\
& & \iou{ 0.0056 \tiny{(-0.2273)} }&\iou{ 0.0548 \tiny{(0.0079)} }&\iou{ 0.0458 \tiny{(-0.2213)} }&\iou{ 0.0159 \tiny{(-0.0146)} }&\iou{ 0.0355 \tiny{(0.0019)} }&\iou{ 0.0199 \tiny{(-0.0283)} }&\iou{ 0.0602 \tiny{(-0.0687)} }&\iou{ 0.0123 \tiny{(-0.0128)} }&\iou{ 0.0520 \tiny{(-0.2853)} }&\iou{ 0.0015 \tiny{(-0.2006)}}\\

& \multirow{2}{*}{\rotatebox[origin=c]{90}{\tiny{RickyG}}} &\mcc{ 0.0241 \tiny{(-0.2986)} }&\mcc{ -0.0243 \tiny{(0.1453)} }&\mcc{ 0.0137 \tiny{(-0.2908)} }&\mcc{ -0.0059 \tiny{(-0.0452)} }&\mcc{ 0.0128 \tiny{(-0.0075)} }&\mcc{ 0.0002 \tiny{(-0.0355)} }&\mcc{ 0.0202 \tiny{(-0.0933)} }&\mcc{ 0.0127 \tiny{(0.0053)} }&\mcc{ 0.0470 \tiny{(-0.3569)} }&\mcc{ -0.0043 \tiny{(-0.2800)}}\\
& &\iou{ 0.0184 \tiny{(-0.2145)} }&\iou{ 0.0536 \tiny{(0.0067)} }&\iou{ 0.0220 \tiny{(-0.2451)} }&\iou{ 0.0143 \tiny{(-0.0162)} }&\iou{ 0.0339 \tiny{(0.0003)} }&\iou{ 0.0287 \tiny{(-0.0196)} }&\iou{ 0.0646 \tiny{(-0.0643)} }&\iou{ 0.0246 \tiny{(-0.0005)} }&\iou{ 0.0592 \tiny{(-0.2781)} }&\iou{ 0.0008 \tiny{(-0.2012)}}\\

\bottomrule
  \end{tabularx}
  \caption{All  datasets \mcc{mcc} and \iou{iou}}
  \label{tab:all-mcc-iou}
\end{table*}

==> tables/coverage-f1.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 24pt}YYYYYYYYYY}

\toprule



 & \textbf{CatNet} & \textbf{CFA} & \textbf{Choi} & \textbf{Comprint} & \textbf{MantraNet} & \textbf{Noiseprint} & \textbf{Shin} & \textbf{SpliceBuster} & \textbf{TruFor} & \textbf{Zero}\\ 
\midrule
\textbf{Original} & 0.2971  & 0.1585  & 0.0184  & 0.1508  & 0.2948  & 0.1512  & 0.1948  & 0.0759  & 0.4864  & 0.1890 \\
\textbf{CameraTE} & 0.1651 \tiny{(-0.1320)} & 0.1593 \tiny{(0.0008)} & 0.0128 \tiny{(-0.0056)} & 0.1263 \tiny{(-0.0245)} & 0.1287 \tiny{(-0.1661)} & 0.1360 \tiny{(-0.0152)} & 0.1846 \tiny{(-0.0102)} & 0.0661 \tiny{(-0.0098)} & 0.3220 \tiny{(-0.1644)} & 0.1830 \tiny{(-0.0060)}\\
\textbf{BM3D} & 0.2934 \tiny{(-0.0037)} & 0.1602 \tiny{(0.0018)} & 0.0065 \tiny{(-0.0120)} & 0.1118 \tiny{(-0.0390)} & 0.1485 \tiny{(-0.1463)} & 0.1379 \tiny{(-0.0133)} & 0.1870 \tiny{(-0.0079)} & 0.0613 \tiny{(-0.0145)} & 0.3879 \tiny{(-0.0985)} & 0.1830 \tiny{(-0.0060)}\\
\textbf{Ricky} & 0.1797 \tiny{(-0.1173)} & 0.1652 \tiny{(0.0067)} & 0.0103 \tiny{(-0.0082)} & 0.1222 \tiny{(-0.0286)} & 0.0961 \tiny{(-0.1987)} & 0.1404 \tiny{(-0.0109)} & 0.1867 \tiny{(-0.0082)} & 0.0692 \tiny{(-0.0067)} & 0.3377 \tiny{(-0.1488)} & 0.0000 \tiny{(-0.1890)}\\
\textbf{RickyG} & 0.2253 \tiny{(-0.0717)} & 0.1571 \tiny{(-0.0014)} & 0.0019 \tiny{(-0.0166)} & 0.1136 \tiny{(-0.0373)} & 0.1248 \tiny{(-0.1700)} & 0.1510 \tiny{(-0.0002)} & 0.1859 \tiny{(-0.0090)} & 0.0609 \tiny{(-0.0149)} & 0.3374 \tiny{(-0.1490)} & 0.0000 \tiny{(-0.1890)}\\




\bottomrule
  \end{tabularx}
  \caption{COVERAGE - F1}
  \label{tab:coverage-f1}
\end{table*}

==> tables/coverage-iou.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 24pt}YYYYYYYYYY}

\toprule


 & \textbf{CatNet} & \textbf{CFA} & \textbf{Choi} & \textbf{Comprint} & \textbf{MantraNet} & \textbf{Noiseprint} & \textbf{Shin} & \textbf{SpliceBuster} & \textbf{TruFor} & \textbf{Zero}\\ 
\midrule
\textbf{Original} & 0.2199  & 0.0879  & 0.0109  & 0.0856  & 0.1856  & 0.0858  & 0.1106  & 0.0423  & 0.3752  & 0.1082 \\
\textbf{CameraTE} & 0.1162 \tiny{(-0.1038)} & 0.0883 \tiny{(0.0003)} & 0.0079 \tiny{(-0.0030)} & 0.0711 \tiny{(-0.0145)} & 0.0719 \tiny{(-0.1137)} & 0.0770 \tiny{(-0.0089)} & 0.1043 \tiny{(-0.0063)} & 0.0361 \tiny{(-0.0062)} & 0.2212 \tiny{(-0.1541)} & 0.1046 \tiny{(-0.0036)}\\
\textbf{BM3D} & 0.2151 \tiny{(-0.0049)} & 0.0891 \tiny{(0.0012)} & 0.0036 \tiny{(-0.0072)} & 0.0617 \tiny{(-0.0240)} & 0.0841 \tiny{(-0.1015)} & 0.0773 \tiny{(-0.0085)} & 0.1055 \tiny{(-0.0051)} & 0.0336 \tiny{(-0.0087)} & 0.2863 \tiny{(-0.0889)} & 0.1046 \tiny{(-0.0036)}\\
\textbf{Ricky} & 0.1278 \tiny{(-0.0922)} & 0.0921 \tiny{(0.0041)} & 0.0059 \tiny{(-0.0050)} & 0.0687 \tiny{(-0.0169)} & 0.0537 \tiny{(-0.1320)} & 0.0790 \tiny{(-0.0068)} & 0.1055 \tiny{(-0.0051)} & 0.0383 \tiny{(-0.0040)} & 0.2427 \tiny{(-0.1325)} & 0.0000 \tiny{(-0.1082)}\\
\textbf{RickyG} & 0.1607 \tiny{(-0.0592)} & 0.0871 \tiny{(-0.0009)} & 0.0010 \tiny{(-0.0099)} & 0.0630 \tiny{(-0.0226)} & 0.0693 \tiny{(-0.1163)} & 0.0858 \tiny{(0.0000)} & 0.1051 \tiny{(-0.0055)} & 0.0334 \tiny{(-0.0090)} & 0.2386 \tiny{(-0.1367)} & 0.0000 \tiny{(-0.1082)}\\





\bottomrule
  \end{tabularx}
  \caption{COVERAGE IoU}
  \label{tab:coverage-iou}
\end{table*}

==> tables/coverage-iqa.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 24pt}YYYYYY}

\toprule

 & \textbf{NIQE} & \textbf{BRISQUE} & \textbf{LPIPS} & \textbf{PSNR} & \textbf{SSIM} & \textbf{SSIM-PYTORCH}\\ 
\midrule
\textbf{Original} & 4.5529 & 19.0256 & 0.0000 & 80.0000 & 1.0000 & 1.0000 \\
\textbf{CameraTE} & 5.4513 & 30.3558 & 0.0631 & 35.7974 & 0.9648 & 0.9112 \\
\textbf{BM3D} & 5.8792 & 35.9560 & 0.0237 & 44.1417 & 0.9888 & 0.9649 \\
\textbf{Ricky} & 4.3343 & 17.1298 & 0.0281 & 33.4959 & 0.9275 & 0.8320 \\
\textbf{RickyG} & 5.0359 & 27.8903 & 0.0276 & 34.6969 & 0.9487 & 0.8878 \\

\bottomrule
  \end{tabularx}
  \caption{COVERAGE - IQA}
  \label{tab:coverage-iqa}
\end{table*}

==> tables/coverage-mcc.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 24pt}YYYYYYYYYY}

\toprule



 & \textbf{CatNet} & \textbf{CFA} & \textbf{Choi} & \textbf{Comprint} & \textbf{MantraNet} & \textbf{Noiseprint} & \textbf{Shin} & \textbf{SpliceBuster} & \textbf{TruFor} & \textbf{Zero}\\ 
\midrule
\textbf{Original} & 0.2747  & -0.0376  & 0.0075  & 0.0230  & 0.2617  & 0.0062  & 0.0615  & -0.0571  & 0.4442  & 0.0326 \\
\textbf{CameraTE} & 0.1480 \tiny{(-0.1267)} & -0.0329 \tiny{(0.0047)} & 0.0056 \tiny{(-0.0020)} & -0.0015 \tiny{(-0.0245)} & 0.0790 \tiny{(-0.1827)} & -0.0230 \tiny{(-0.0292)} & 0.0489 \tiny{(-0.0127)} & -0.0722 \tiny{(-0.0151)} & 0.2614 \tiny{(-0.1828)} & 0.0238 \tiny{(-0.0088)}\\
\textbf{BM3D} & 0.2666 \tiny{(-0.0081)} & -0.0415 \tiny{(-0.0039)} & 0.0051 \tiny{(-0.0024)} & -0.0281 \tiny{(-0.0511)} & 0.0371 \tiny{(-0.2246)} & -0.0145 \tiny{(-0.0207)} & 0.0515 \tiny{(-0.0100)} & -0.0771 \tiny{(-0.0200)} & 0.3267 \tiny{(-0.1175)} & 0.0236 \tiny{(-0.0091)}\\
\textbf{Ricky} & 0.1598 \tiny{(-0.1149)} & -0.0238 \tiny{(0.0138)} & 0.0011 \tiny{(-0.0064)} & -0.0065 \tiny{(-0.0295)} & 0.0483 \tiny{(-0.2133)} & -0.0115 \tiny{(-0.0176)} & 0.0514 \tiny{(-0.0101)} & -0.0602 \tiny{(-0.0031)} & 0.2849 \tiny{(-0.1594)} & 0.0000 \tiny{(-0.0326)}\\
\textbf{RickyG} & 0.2003 \tiny{(-0.0745)} & -0.0405 \tiny{(-0.0029)} & -0.0004 \tiny{(-0.0079)} & -0.0124 \tiny{(-0.0354)} & 0.0680 \tiny{(-0.1937)} & 0.0024 \tiny{(-0.0038)} & 0.0475 \tiny{(-0.0140)} & -0.0717 \tiny{(-0.0146)} & 0.2738 \tiny{(-0.1704)} & 0.0000 \tiny{(-0.0326)}\\




\bottomrule
  \end{tabularx}
  \caption{COVERAGE MCC}
  \label{tab:coverage-mcc}
\end{table*}

==> tables/fau-f1.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 24pt}YYYYYYYYYY}

\toprule

 & \textbf{CatNet} & \textbf{Bammey} & \textbf{Choi} & \textbf{Comprint} & \textbf{MantraNet} & \textbf{Noiseprint} & \textbf{Shin} & \textbf{SpliceBuster} & \textbf{TruFor} & \textbf{Zero}\\ 
\midrule
\textbf{Original} & 0.3187  & 0.0827  & 0.3122  & 0.0566  & 0.0630  & 0.0888  & 0.1843  & 0.0471  & 0.4203  & 0.2958 \\
\textbf{CameraTE} & 0.0159 \tiny{(-0.3027)} & 0.0909 \tiny{(0.0082)} & 0.1496 \tiny{(-0.1626)} & 0.0376 \tiny{(-0.0190)} & 0.0787 \tiny{(0.0157)} & 0.0806 \tiny{(-0.0082)} & 0.1639 \tiny{(-0.0204)} & 0.0517 \tiny{(0.0045)} & 0.1008 \tiny{(-0.3196)} & 0.1089 \tiny{(-0.1870)}\\
\textbf{BM3D} & 0.0741 \tiny{(-0.2446)} & 0.0911 \tiny{(0.0084)} & 0.0722 \tiny{(-0.2399)} & 0.0237 \tiny{(-0.0328)} & 0.0690 \tiny{(0.0060)} & 0.0606 \tiny{(-0.0282)} & 0.1298 \tiny{(-0.0545)} & 0.0460 \tiny{(-0.0012)} & 0.1287 \tiny{(-0.2917)} & 0.1012 \tiny{(-0.1946)}\\
\textbf{Ricky} & 0.0099 \tiny{(-0.3088)} & 0.0973 \tiny{(0.0146)} & 0.0781 \tiny{(-0.2341)} & 0.0294 \tiny{(-0.0271)} & 0.0643 \tiny{(0.0013)} & 0.0383 \tiny{(-0.0505)} & 0.1061 \tiny{(-0.0781)} & 0.0238 \tiny{(-0.0233)} & 0.0935 \tiny{(-0.3269)} & 0.0027 \tiny{(-0.2931)}\\
\textbf{RickyG} & 0.0301 \tiny{(-0.2886)} & 0.0953 \tiny{(0.0126)} & 0.0318 \tiny{(-0.2804)} & 0.0275 \tiny{(-0.0291)} & 0.0630 \tiny{(-0.0000)} & 0.0544 \tiny{(-0.0344)} & 0.1109 \tiny{(-0.0733)} & 0.0450 \tiny{(-0.0021)} & 0.1051 \tiny{(-0.3153)} & 0.0016 \tiny{(-0.2942)}\\


\bottomrule
  \end{tabularx}
  \caption{FAU-F1}
  \label{tab:fau-f1}
\end{table*}

==> tables/fau-iou.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 24pt}YYYYYYYYYY}

\toprule



 & \textbf{CatNet} & \textbf{Bammey} & \textbf{Choi} & \textbf{Comprint} & \textbf{MantraNet} & \textbf{Noiseprint} & \textbf{Shin} & \textbf{SpliceBuster} & \textbf{TruFor} & \textbf{Zero}\\ 
\midrule
\textbf{Original} & 0.2329  & 0.0469  & 0.2670  & 0.0305  & 0.0336  & 0.0482  & 0.1289  & 0.0251  & 0.3373  & 0.2021 \\
\textbf{CameraTE} & 0.0085 \tiny{(-0.2244)} & 0.0516 \tiny{(0.0047)} & 0.1173 \tiny{(-0.1497)} & 0.0206 \tiny{(-0.0099)} & 0.0427 \tiny{(0.0091)} & 0.0434 \tiny{(-0.0049)} & 0.1046 \tiny{(-0.0243)} & 0.0277 \tiny{(0.0026)} & 0.0572 \tiny{(-0.2801)} & 0.0633 \tiny{(-0.1388)}\\
\textbf{BM3D} & 0.0517 \tiny{(-0.1812)} & 0.0517 \tiny{(0.0048)} & 0.0559 \tiny{(-0.2111)} & 0.0126 \tiny{(-0.0179)} & 0.0377 \tiny{(0.0041)} & 0.0331 \tiny{(-0.0152)} & 0.0803 \tiny{(-0.0486)} & 0.0243 \tiny{(-0.0008)} & 0.0799 \tiny{(-0.2574)} & 0.0583 \tiny{(-0.1438)}\\
\textbf{Ricky} & 0.0056 \tiny{(-0.2273)} & 0.0548 \tiny{(0.0079)} & 0.0458 \tiny{(-0.2213)} & 0.0159 \tiny{(-0.0146)} & 0.0355 \tiny{(0.0019)} & 0.0199 \tiny{(-0.0283)} & 0.0602 \tiny{(-0.0687)} & 0.0123 \tiny{(-0.0128)} & 0.0520 \tiny{(-0.2853)} & 0.0015 \tiny{(-0.2006)}\\
\textbf{RickyG} & 0.0184 \tiny{(-0.2145)} & 0.0536 \tiny{(0.0067)} & 0.0220 \tiny{(-0.2451)} & 0.0143 \tiny{(-0.0162)} & 0.0339 \tiny{(0.0003)} & 0.0287 \tiny{(-0.0196)} & 0.0646 \tiny{(-0.0643)} & 0.0246 \tiny{(-0.0005)} & 0.0592 \tiny{(-0.2781)} & 0.0008 \tiny{(-0.2012)}\\




\bottomrule
  \end{tabularx}
  \caption{FAU IoU}
  \label{tab:fau-iou}
\end{table*}

==> tables/fau-iqa.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 24pt}YYYYYY}

\toprule

 & \textbf{NIQE} & \textbf{BRISQUE} & \textbf{LPIPS} & \textbf{PSNR} & \textbf{SSIM} & \textbf{SSIM-PYTORCH}\\ 
\midrule
\textbf{Original} & 4.7392 & 20.5726 & 0.0000 & 80.0000 & 1.0000 & 1.0000 \\
\textbf{CameraTE} & 5.8360 & 40.1577 & 0.2098 & 37.8765 & 0.9460 & 0.8352 \\
\textbf{BM3D} & 5.4875 & 42.7470 & 0.1045 & 41.2625 & 0.9797 & 0.9226 \\
\textbf{Ricky} & 3.8896 & 19.8268 & 0.0985 & 33.0308 & 0.8792 & 0.6840 \\
\textbf{RickyG} & 4.2440 & 29.9920 & 0.0952 & 34.4725 & 0.9159 & 0.7842 \\

\bottomrule
  \end{tabularx}
  \caption{FAU - IQA}
  \label{tab:fau-iqa}
\end{table*}

==> tables/fau-mcc.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 24pt}YYYYYYYYYY}

\toprule



 & \textbf{CatNet} & \textbf{Bammey} & \textbf{Choi} & \textbf{Comprint} & \textbf{MantraNet} & \textbf{Noiseprint} & \textbf{Shin} & \textbf{SpliceBuster} & \textbf{TruFor} & \textbf{Zero}\\ 
\midrule
\textbf{Original} & 0.3228  & -0.1696  & 0.3045  & 0.0393  & 0.0203  & 0.0358  & 0.1134  & 0.0074  & 0.4039  & 0.2757 \\
\textbf{CameraTE} & 0.0141 \tiny{(-0.3087)} & -0.0738 \tiny{(0.0958)} & 0.1426 \tiny{(-0.1620)} & 0.0092 \tiny{(-0.0302)} & 0.0154 \tiny{(-0.0049)} & 0.0242 \tiny{(-0.0116)} & 0.0826 \tiny{(-0.0308)} & 0.0045 \tiny{(-0.0029)} & 0.0553 \tiny{(-0.3486)} & -0.0010 \tiny{(-0.2767)}\\
\textbf{BM3D} & 0.0757 \tiny{(-0.2471)} & -0.0692 \tiny{(0.1004)} & 0.0679 \tiny{(-0.2367)} & -0.0017 \tiny{(-0.0410)} & -0.0268 \tiny{(-0.0470)} & -0.0014 \tiny{(-0.0372)} & 0.0411 \tiny{(-0.0723)} & 0.0011 \tiny{(-0.0064)} & 0.0802 \tiny{(-0.3237)} & -0.0114 \tiny{(-0.2871)}\\
\textbf{Ricky} & 0.0070 \tiny{(-0.3157)} & -0.0130 \tiny{(0.1567)} & 0.0242 \tiny{(-0.2803)} & 0.0001 \tiny{(-0.0392)} & 0.0057 \tiny{(-0.0146)} & -0.0018 \tiny{(-0.0376)} & 0.0128 \tiny{(-0.1006)} & -0.0050 \tiny{(-0.0124)} & 0.0399 \tiny{(-0.3640)} & -0.0007 \tiny{(-0.2765)}\\
\textbf{RickyG} & 0.0241 \tiny{(-0.2986)} & -0.0243 \tiny{(0.1453)} & 0.0137 \tiny{(-0.2908)} & -0.0059 \tiny{(-0.0452)} & 0.0128 \tiny{(-0.0075)} & 0.0002 \tiny{(-0.0355)} & 0.0202 \tiny{(-0.0933)} & 0.0127 \tiny{(0.0053)} & 0.0470 \tiny{(-0.3569)} & -0.0043 \tiny{(-0.2800)}\\




\bottomrule
  \end{tabularx}
  \caption{FAU MCC}
  \label{tab:fau-mcc}
\end{table*}

==> tables/korus-f1.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
  \setlength{\tabcolsep}{1em}

\begin{table*}[h]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 2pt}YYYYYYYYYY}

\toprule

 & CatNet & Bammey \etal & Choi & Comprint & MantraNet & Noiseprint & Shin & Splicebuster & TruFor & Zero\\ 
\midrule
Original & 0.0657  & 0.0825  & 0.1717  & 0.0817  & 0.1607  & 0.1389  & 0.1035  & 0.1682  & 0.3473  & 0.0043 \\
CamTE & 0.0420 \tiny{(-0.0237)} & 0.0833 \tiny{(0.0009)} & 0.0562 \tiny{(-0.1155)} & 0.0710 \tiny{(-0.0107)} & 0.1147 \tiny{(-0.0460)} & 0.0987 \tiny{(-0.0402)} & 0.1059 \tiny{(0.0024)} & 0.1261 \tiny{(-0.0422)} & 0.2246 \tiny{(-0.1227)} & 0.0000 \tiny{(-0.0043)}\\
BM3D & 0.0937 \tiny{(0.0280)} & 0.0877 \tiny{(0.0053)} & 0.0314 \tiny{(-0.1403)} & 0.0634 \tiny{(-0.0184)} & 0.1278 \tiny{(-0.0329)} & 0.0939 \tiny{(-0.0450)} & 0.0987 \tiny{(-0.0048)} & 0.1274 \tiny{(-0.0409)} & 0.2803 \tiny{(-0.0670)} & 0.0000 \tiny{(-0.0043)}\\
\textit{Diff-CF} & 0.0324 \tiny{(-0.0333)} & 0.0931 \tiny{(0.0106)} & 0.0440 \tiny{(-0.1278)} & 0.0398 \tiny{(-0.0419)} & 0.0769 \tiny{(-0.0838)} & 0.0669 \tiny{(-0.0720)} & 0.0903 \tiny{(-0.0131)} & 0.0720 \tiny{(-0.0963)} & 0.1841 \tiny{(-0.1631)} & 0.0046 \tiny{(0.0003)}\\
\textit{Diff-CFG} & 0.0775 \tiny{(0.0118)} & 0.0912 \tiny{(0.0087)} & 0.0077 \tiny{(-0.1640)} & 0.0520 \tiny{(-0.0298)} & 0.0980 \tiny{(-0.0627)} & 0.0816 \tiny{(-0.0573)} & 0.0910 \tiny{(-0.0125)} & 0.0852 \tiny{(-0.0831)} & 0.2398 \tiny{(-0.1074)} & 0.0019 \tiny{(-0.0024)}\\



\bottomrule
  \end{tabularx}
  \caption{F1 scores obtained for all the tested methods on the Korus dataset~\cite{korus1, korus2}.}
  \label{tab:korus-f1}

\end{table*}

==> tables/korus-iou.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

  \setlength{\tabcolsep}{1em}

\begin{table*}[h]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 2pt}YYYYYYYYYY}

\toprule

 & CatNet & Bammey \etal & Choi & Comprint & MantraNet & Noiseprint & Shin & Splicebuster & TruFor & Zero\\ 
\midrule
Original & 0.0433  & 0.0446  & 0.1261  & 0.0461  & 0.0982  & 0.0792  & 0.0568  & 0.1012  & 0.2575  & 0.0028 \\
CamTE & 0.0278 \tiny{(-0.0155)} & 0.0452 \tiny{(0.0005)} & 0.0400 \tiny{(-0.0860)} & 0.0389 \tiny{(-0.0072)} & 0.0644 \tiny{(-0.0338)} & 0.0545 \tiny{(-0.0247)} & 0.0578 \tiny{(0.0011)} & 0.0729 \tiny{(-0.0284)} & 0.1489 \tiny{(-0.1086)} & 0.0000 \tiny{(-0.0028)}\\
BM3D & 0.0646 \tiny{(0.0213)} & 0.0478 \tiny{(0.0031)} & 0.0227 \tiny{(-0.1033)} & 0.0346 \tiny{(-0.0115)} & 0.0746 \tiny{(-0.0237)} & 0.0514 \tiny{(-0.0278)} & 0.0540 \tiny{(-0.0028)} & 0.0744 \tiny{(-0.0268)} & 0.1964 \tiny{(-0.0611)} & 0.0000 \tiny{(-0.0028)}\\
\textit{Diff-CF} & 0.0204 \tiny{(-0.0229)} & 0.0505 \tiny{(0.0059)} & 0.0246 \tiny{(-0.1014)} & 0.0215 \tiny{(-0.0246)} & 0.0416 \tiny{(-0.0566)} & 0.0360 \tiny{(-0.0432)} & 0.0487 \tiny{(-0.0081)} & 0.0401 \tiny{(-0.0611)} & 0.1131 \tiny{(-0.1445)} & 0.0027 \tiny{(-0.0001)}\\
\textit{Diff-CFG} & 0.0527 \tiny{(0.0095)} & 0.0495 \tiny{(0.0048)} & 0.0043 \tiny{(-0.1217)} & 0.0281 \tiny{(-0.0180)} & 0.0552 \tiny{(-0.0430)} & 0.0446 \tiny{(-0.0346)} & 0.0491 \tiny{(-0.0076)} & 0.0488 \tiny{(-0.0525)} & 0.1601 \tiny{(-0.0975)} & 0.0011 \tiny{(-0.0017)}\\



\bottomrule
  \end{tabularx}
  \caption{IoU scores obtained for all the tested methods (including Bammey~\etal) on the Korus dataset~\cite{korus1, korus2}.}
  \label{tab:korus-iou}
\end{table*}

==> tables/korus-iqa.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 24pt}YYYYYY}

\toprule

 & \textbf{NIQE} & \textbf{BRISQUE} & \textbf{LPIPS} & \textbf{PSNR} & \textbf{SSIM} & \textbf{SSIM-PYTORCH}\\ 
\midrule
\textbf{Original} & 5.7271 & 13.7602 & 0.0000 & 80.0000 & 1.0000 & 1.0000 \\
\textbf{CameraTE} & 5.5442 & 34.5632 & 0.1684 & 38.2833 & 0.9433 & 0.8672 \\
\textbf{BM3D} & 5.1004 & 38.0418 & 0.0835 & 43.1409 & 0.9802 & 0.9368 \\
\textbf{Ricky} & 3.8693 & 23.1161 & 0.0733 & 32.9680 & 0.8769 & 0.7238 \\
\textbf{RickyG} & 4.1070 & 28.3290 & 0.0771 & 34.3391 & 0.9126 & 0.8104 \\

\bottomrule
  \end{tabularx}
  \caption{KORUS - IQA}
  \label{tab:korus-iqa}
\end{table*}

==> tables/korus-mcc.tex <==
% \newcolumntype{Y}{>{\centering\arraybackslash}X}

  \setlength{\tabcolsep}{0.7em}

\begin{table*}[t]  
  \small  
  \centering
  \begin{tabularx}{1\textwidth}{c@{\hskip 2pt}YYYYYYYYYY}

\toprule

 & CatNet & Bammey \etal & Choi & Comprint & MantraNet & Noiseprint & Shin & Splicebuster & TruFor & Zero\\ 
\midrule
Original & 0.0790  & -0.1548  & 0.1971  & 0.0534  & 0.1261  & 0.0988  & 0.0221  & 0.1405  & 0.3428  & 0.0050 \\
CamTE & 0.0468 \tiny{(-0.0322)} & -0.0608 \tiny{(0.0940)} & 0.0597 \tiny{(-0.1374)} & 0.0356 \tiny{(-0.0179)} & 0.0646 \tiny{(-0.0614)} & 0.0420 \tiny{(-0.0569)} & 0.0305 \tiny{(0.0084)} & 0.0817 \tiny{(-0.0588)} & 0.1961 \tiny{(-0.1467)} & 0.0000 \tiny{(-0.0050)}\\
BM3D & 0.0997 \tiny{(0.0207)} & -0.0452 \tiny{(0.1095)} & 0.0352 \tiny{(-0.1619)} & 0.0278 \tiny{(-0.0256)} & 0.0652 \tiny{(-0.0609)} & 0.0420 \tiny{(-0.0569)} & 0.0155 \tiny{(-0.0066)} & 0.0860 \tiny{(-0.0545)} & 0.2579 \tiny{(-0.0850)} & 0.0000 \tiny{(-0.0050)}\\
\textit{Diff-CF} & 0.0418 \tiny{(-0.0371)} & -0.0030 \tiny{(0.1518)} & 0.0147 \tiny{(-0.1825)} & 0.0024 \tiny{(-0.0510)} & 0.0255 \tiny{(-0.1005)} & 0.0190 \tiny{(-0.0798)} & 0.0027 \tiny{(-0.0194)} & 0.0350 \tiny{(-0.1055)} & 0.1454 \tiny{(-0.1974)} & 0.0045 \tiny{(-0.0005)}\\
\textit{Diff-CFG} & 0.0852 \tiny{(0.0063)} & -0.0096 \tiny{(0.1452)} & 0.0044 \tiny{(-0.1927)} & 0.0125 \tiny{(-0.0409)} & 0.0442 \tiny{(-0.0818)} & 0.0267 \tiny{(-0.0722)} & 0.0040 \tiny{(-0.0181)} & 0.0456 \tiny{(-0.0950)} & 0.2064 \tiny{(-0.1364)} & 0.0005 \tiny{(-0.0045)}\\







\bottomrule
  \end{tabularx}
  \caption{MCC scores obtained for all the tested methods (including Bammey~\etal) on the Korus dataset~\cite{korus1, korus2}.}
  \label{tab:Korus-MCC}
\end{table*}
